Process Dimension of Classical and Non-Commutative Processes

We treat observable operator models (OOM) and their non-commutative generalisation, which we call NC-OOMs. A natural characteristic of a stochastic process in the context of classical OOM theory is the process dimension. We investigate its properties within the more general formulation, which allows to consider process dimension as a measure of complexity of non-commutative processes: We prove lower semi-continuity, and derive an ergodic decomposition formula. Further, we obtain results on the close relationship between the canonical OOM and the concept of causal states which underlies the definition of statistical complexity. In particular, the topological statistical complexity, i.e. the logarithm of the number of causal states, turns out to be an upper bound to the logarithm of process dimension.

==> Makefile <==
NAME=prozessdim
VERSION=4.6

SHELL=/bin/bash

TEXFILES=$(NAME).tex intro.tex oom.tex infinite-past.tex noncomut.tex results.tex macros.tex format-short.sty wollatex.sty
FILES=$(TEXFILES) bib-math.bib Makefile version

.PHONY: print tar untar backup pdf default dvi clean new


default:	dvi
print:		printed
dvi:		$(NAME).dvi
pdf:		$(NAME).pdf
new:		clean dvi

tar:;		echo -n $(VERSION) > version
		tar -chf $(NAME).tar $(FILES)
		gzip -f $(NAME).tar
		mv $(NAME).tar.gz $(NAME)-$(VERSION)-`date '+%Y.%m.%d'`.tar.gz

untar:;		tarname=`echo *.tar.gz`; \
			if [ `echo $$tarname | wc -w` -gt 1 ]; then echo "multiple tar files!"; exit 1; \
			else gunzip $$tarname && tar -xf $${tarname%.gz} && gzip $${tarname%.gz}; fi

backup:		dvi	
		tar -chf $(NAME).tar $(FILES)
		gzip -f $(NAME).tar
		datum=`date '+%Y.%m.%d'`; mv -i $(NAME).tar.gz backup/$(NAME)-$(VERSION)-$$datum.tar.gz && \
		cp -i $(NAME).dvi backup/$(NAME)-$(VERSION)-$$datum.dvi;

printed:	$(NAME).dvi
		echo -n "really print (y/n)? "; \
		read answer; if [ "$$answer" = "y" ]; then dvips $(NAME).dvi && touch printed; else echo "Aborted!"; fi

$(NAME).dvi:	$(TEXFILES)
		echo -n $(VERSION) > version
		latex $(NAME)
		if grep '\\citation' $(NAME).aux > /dev/null; then bibtex $(NAME); fi
		latex $(NAME)
		latex $(NAME)

$(NAME).pdf:	$(NAME).dvi $(TEXFILES)
		dvips -ta4 -o $(NAME).ps $(NAME).dvi
		ps2pdf $(NAME).ps

clean:;		rm -f `eval echo $(NAME).{aux,bbl,blg,log,toc,dvi,ps,pdf}`


